Recover and Identify: A Generative Dual Model for Cross-Resolution Person Re-Identification

Person re-identification (re-ID) aims at matching images of the same identity across camera views. Due to varying distances between cameras and persons of interest, resolution mismatch can be expected, which would degrade person re-ID performance in real-world scenarios. To overcome this problem, we propose a novel generative adversarial network to address cross-resolution person re-ID, allowing query images with varying resolutions. By advancing adversarial learning techniques, our proposed model learns resolution-invariant image representations while being able to recover the missing details in low-resolution input images. The resulting features can be jointly applied for improving person re-ID performance due to preserving resolution invariance and recovering re-ID oriented discriminative details. Our experiments on five benchmark datasets confirm the effectiveness of our approach and its superiority over the state-of-the-art methods, especially when the input resolutions are unseen during training.

==> comparison.tex <==
\begin{table}[t]
  \scriptsize
  \caption{Experimental results of cross-resolution person re-ID with seen and unseen resolutions on the MLR-VIPeR dataset evaluated at rank 1.}
  \vspace{\tablecapmargin}
  \centering
  \label{table:comparison}
  \resizebox{\linewidth}{!}
  {
  \begin{tabular}{l|l|ccc}
  %
  \toprule
  %
  \multirow{2}{*}{Train} & \multirow{2}{*}{Test} & \multicolumn{3}{c}{MLR-VIPeR} \\
  %
  & & SING & CSR-GAN & Ours \\
  %
  \midrule
  %
  $r \in \{1, 2, 3, 4\}$ & $r \in \{2, 3, 4\}$ & 33.5 & 37.2 & 42.5 \\
  %
%   $r \in \{1, 2, 4\}$  & $r \in \{2, 3, 4\}$ & \xmark & \xmark & 42.3 \\
  %
  $r \in \{1, 2, 3, 4\}$  & $r = 8$ & \xmark & \xmark & 37.5 \\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \vspace{2.0\tablemargin}
\end{table}

==> exp/dataset.tex <==
\begin{table}[t]
  \small
  \ra{1.3}
  \begin{center}
  \caption{Statistics of the adopted datasets.}
  %
  \vspace{\tablecapmargin}
  \label{table:dataset-stat}
  \resizebox{1\linewidth}{!} 
  {
  \begin{tabular}{l|ccc|c}
  %
  \toprule
  %
  \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Statistics} & \multirow{2}{*}{Down-sampling} \\
  %
   & \# of images & \#  of cameras & \# of identities &\\
  %
  \midrule
  %
  MLR-CUHK03 & 14000 & 5 & 1467 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  MLR-ViPeR & 1264 & 2 & 632 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  CAVIAR & 1220 & 2 & 72 & \xmark \\
  %
  MLR-Market-1501 & 32668 & 6 & 1501 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  MLR-DukeMTMC-reID & 36411 & 8 & 1404 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  \midrule
  %
  Market-1501 & 32668 & 6 & 1501 & \xmark \\
  %
  DukeMTMC-reID & 36411 & 8 & 1404 & \xmark \\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{-2.0mm}
\end{table}

==> exp/exp-LR.tex <==
%
\begin{table}[h]
  \small
  \ra{1.3}
  \begin{center}
  \caption{Train multi-scale LR images and test on lowest resolution images.}
  %\vspace{\tablecapmargin}
  \label{table:exp-LR}
  \resizebox{\linewidth}{!} 
  {
  \begin{tabular}{l|l|l|ccccc}
  %
  \toprule
  %
  \multirow{2}{*}{Train} & \multirow{2}{*}{Test} & \multirow{2}{*}{Method} & \multicolumn{5}{c}{CUHK03} \\
  %
  & & & Rank 1 & Rank 5 & Rank 10 & Rank 20 & mAP \\
  %
  \midrule
  %
  \multirow{2}{*}{D=4} & \multirow{2}{*}{D=4} & Ours (single-level) & 71.3 & 94.1 & 97.9 & 99.4 & 66.9 \\
  %
  & & Ours (single-level RK) & 83.2 & 96.3 & 98.6 & 99.5 & 80.7 \\
  %
  \midrule
  %
  \multirow{2}{*}{D=2,3,4} & \multirow{2}{*}{D=4} & Ours (single-level) & 73.0 & 94.7 & 98.0 & 99.3 & 69.8 \\
  %
  & & Ours (single-level RK) & 81.3 & 96.0 & 98.3 & 99.4 & 79.1 \\
  %
  \midrule
  %
  \multirow{2}{*}{D=8} & \multirow{2}{*}{D=8} & Ours (single-level) & 55.6 & 86.1 & 92.8 & 97.3 & 51.0 \\
  %
  & & Ours (single-level RK) & 66.7 & 89.3 & 93.9 & 97.5 & 63.2 \\
  %
  \midrule
  %
  \multirow{2}{*}{D=2,4,8} & \multirow{2}{*}{D=8} & Ours (single-level) & 62.7 & 90.7 & 96.2 & 98.8 & 58.5 \\
  %
  & & Ours (single-level RK) & 73.6 & 92.7 & 96.7 & 98.9 & 70.4 \\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{\tablemargin}
\end{table}

==> exp/exp-multi-Re.tex <==
%
\begin{table}[t]
  \small
  \ra{1.3}
  \begin{center}
  \caption{Effect of training images of multiple low resolutions. The bold numbers indicate the best results.}
  \vspace{\tablecapmargin}
  \label{table:exp-multi-resolution}
  \resizebox{\linewidth}{!} 
  {
  \begin{tabular}{ll|cc|cc|cc}
  %
  \toprule
  %
  \multicolumn{2}{l|}{Train} & \multicolumn{2}{c|}{MLR-CUHK03} & \multicolumn{2}{c|}{MLR-VIPeR} & \multicolumn{2}{c}{CAVIAR} \\
  %
  HR & LR & Rank 1 & mAP & Rank 1 & mAP & Rank 1 & mAP \\
  %
  \midrule
  %
  $r = 1$ & $r = 2$ & 70.9 & 67.7 & 38.9 & 42.6 & 36.3 & 52.9\\
  %
  $r = 1$ & $r = 3$ & 72.3 & 68.8 & 40.3 & 43.2 & 37.9 & 53.1\\
  %
  $r = 1$ & $r = 4$ & 77.2 &74.8 & 41.5 & 45.4 & 40.1 & 54.6\\
  %
  $r = 1$ & $r \in \{2, 3, 4\}$ & \textbf{78.9} & \textbf{75.9} & \textbf{42.5}& \textbf{47.0}& \textbf{42.0}& \textbf{56.3}\\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{2.0\tablemargin}
\end{table}

==> exp/recovery.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/uni.png}
  \vspace{-1.0mm}
  \caption{\textbf{Recovered HR images on the MLR-CUHK03 test set.} Given images of the same identity with eight different down-sampling rates, we present the corresponding HR images recovered by our CRGAN.}
  \label{fig:HR-uni}
  \vspace{-5.0mm}
\end{figure}

==> exp/standard_reID.tex <==
\begin{table}[!tbp]
  \small
  \ra{1.3}
  \begin{center}
  \caption{\textbf{Results of standard re-ID (\%).} All methods employ the same feature backbone (\ie ResNet-$50$). Bold and underlined numbers indicate top two results, respectively.}
  %
  \vspace{-2.5mm}
  \label{table:exp-standard-reid}
  \resizebox{0.88\linewidth}{!} 
  {
  \begin{tabular}{l|cc|cc}
  %
  \toprule
  %
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Market-1501} & \multicolumn{2}{c}{DukeMTMC-reID} \\
  %
  & Rank 1 & mAP & Rank 1 & mAP\\
  %
  \midrule
  %
  SVDNet~\cite{sun2017svdnet} & 82.3 & 62.1 & 76.7 & 56.8 \\
  %
  CamStyle~\cite{zhong2017camera} & 89.2 &  71.6 & 78.6  &  57.6 \\
  %
  PN-GAN~\cite{qian2017pose} & 89.4 & 72.6 & 73.6 &  53.2 \\
  %
  FD-GAN~\cite{ge2018fd} & \underline{90.5} & \underline{77.7} & \underline{80.0} &  \underline{64.5} \\
  %
  \midrule
  %
  Ours & \bf{91.5} & \bf{78.1} & \bf{81.8} & \bf{65.6} \\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{-7.5mm}
\end{table}

==> exp/visual_intro.tex <==
\setlength{\fiveimg}{0.1\linewidth}
\begin{figure*}[t]
  \ra{1.3}
  \centering
  \begin{subfigure}[b]{\dimexpr\fiveimg+12pt\relax}
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize Baseline }}}%
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize (Train on HR)}}}%
    \includegraphics[width=0.95\fiveimg,cfbox=white 1pt 1pt]{rank-sample/Q_8.png}\\
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize Baseline (Train}}}%
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize on HR \& LR)}}}%
    \includegraphics[width=0.95\fiveimg,cfbox=white 1pt 1pt]{rank-sample/Q_8.png}\\
    \makebox[12pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize Ours}}}%
    \includegraphics[width=0.95\fiveimg,cfbox=white 1pt 1pt]{rank-sample/Q_8.png}\\
    \vspace{\figmargin}
    \caption*{\hspace{5mm}\scriptsize Query}
  \end{subfigure}
  %
  \hskip .1em
  \vrule
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/403.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/557.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/407.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 1}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/408.png}\\ 
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/408.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/402.png}\\
    \vspace{\figmargin} 
    \caption*{\scriptsize Top 2}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/703.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/403.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/411.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 3}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/402.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/411.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/404.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 4}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/549.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/406.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/409.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 5}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/564.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/402.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/406.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 6}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/700.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/565.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/408.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 7}
  \end{subfigure}
  %
  \caption{Example of the top-ranked HR gallery images of the MLR-CUHK03 dataset which are matched by the LR query input. Images bounded in green and red rectangles denote correct and incorrect matches, respectively.}
  %
  \vspace{0.8\figmargin}
  \label{fig:rank}
\end{figure*}



==> semi-supervised.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{img/semi.pdf}
  \vspace{\figcapmargin}
  \caption{Semi-supervised cross-resolution person re-ID on the MLR-CUHK03 dataset.}
  \label{fig:exp-semi}
  \vspace{\figmargin}
\end{figure}
